High-Order Mixed Finite Element Variable Eddington Factor Methods

We apply high-order mixed finite element discretization techniques and their associated preconditioned iterative solvers to the Variable Eddington Factor (VEF) equations in two spatial dimensions. The mixed finite element VEF discretizations are coupled to a high-order Discontinuous Galerkin (DG) discretization of the Discrete Ordinates transport equation to form effective linear transport algorithms that are compatible with high-order (curved) meshes. This combination of VEF and transport discretizations is motivated by the use of high-order mixed finite element methods in hydrodynamics calculations at the Lawrence Livermore National Laboratory. Due to the mathematical structure of the VEF equations, the standard Raviart Thomas (RT) mixed finite elements cannot be used to approximate the vector variable in the VEF equations. Instead, we investigate three alternatives based on the use of continuous finite elements for each vector component, a non-conforming RT approach where DG-like techniques are used, and a hybridized RT method. We present numerical results that demonstrate high-order accuracy, compatibility with curved meshes, and robust and efficient convergence in iteratively solving the coupled transport-VEF system and in the preconditioned linear solvers used to invert the discretized VEF equations.

==> Makefile <==
# command to use to run python 
PYTHON = python3

# location of figures 
figdir = figs
# location of python source files 
PYSRC = pysrc
# location of data files 
datadir = data
# location of tikz files 
tikzdir = tikz

# location of matplotlibrc (makes plots look nice) 
MPL = matplotlibrc

REF = references.bib

# name of main document 
MAIN = doc

# list of figures to be built for the document 
FIGS = elo_h1 elo_rt elo_hrt elo3p_h1 elo3p_rt elo3p_hrt curved\
hyb_sparsity pts_lineout
FIGS := $(addsuffix .pdf, $(FIGS))

# list of tables to build
TABS = mms mms_elev mms_diff eps_table solvers cp weak
TABS := $(addsuffix .tex, $(TABS))
TABS := $(addprefix $(figdir)/, $(TABS))

TIKZ = $(notdir $(basename $(wildcard $(tikzdir)/*.tex)))
TIKZ := $(addsuffix .pdf, $(TIKZ))

# search for .py dependencies in SRC directory 
vpath %.py $(PYSRC)
# also search for .pdf in figdir 
vpath %.pdf $(figdir)
# search for .tex dependencies in tikzdir 
vpath %.tex $(tikzdir) 

# generate figures, tables, and latex document 
.PHONY : all 
all : $(MAIN).pdf

$(figdir) : 
	mkdir -p $(figdir)

# make figures from python code. save to figdir directory 
%.pdf : %.py $(MPL) $(datadir)/*
	$(PYTHON) $< $(figdir)/$@

# build tables from corresponding python code 
$(figdir)/%.tex : %.py $(datadir)/*
	$(PYTHON) $< $@ 

$(figdir)/mms.tex : mms.py $(datadir)/mms/*
	$(PYTHON) $< $@ $(datadir)/mms/
$(figdir)/mms_elev.tex : mms.py $(datadir)/mms_elev/*
	$(PYTHON) $< $@ $(datadir)/mms_elev/
$(figdir)/mms_diff.tex : mms.py $(datadir)/mms_diff/*
	$(PYTHON) $< $@ $(datadir)/mms_diff/

elo_h1.pdf : eps_lineout.py $(MPL) $(datadir)/tdl_orthog/*
	$(PYTHON) $< $(figdir)/$@ data/tdl_orthog/h1
elo_rt.pdf : eps_lineout.py $(MPL) $(datadir)/tdl_orthog/* 
	$(PYTHON) $< $(figdir)/$@ data/tdl_orthog/rt
elo_hrt.pdf : eps_lineout.py $(MPL) $(datadir)/tdl_orthog/* 
	$(PYTHON) $< $(figdir)/$@ data/tdl_orthog/hrt
elo3p_h1.pdf : eps_lineout.py $(MPL) $(datadir)/tdl_3p/* 
	$(PYTHON) $< $(figdir)/$@ data/tdl_3p/h1 1
elo3p_rt.pdf : eps_lineout.py $(MPL) $(datadir)/tdl_3p/* 
	$(PYTHON) $< $(figdir)/$@ data/tdl_3p/rt 1
elo3p_hrt.pdf : eps_lineout.py $(MPL) $(datadir)/tdl_3p/* 
	$(PYTHON) $< $(figdir)/$@ data/tdl_3p/hrt 1

# weak scaling efficiency table/plot 
$(figdir)/weak.tex : weak.py $(MPL) $(datadir)/yweak/* 
	$(PYTHON) $< $@ $(figdir)/weak_eff.pdf 

# build standalone TIKZ figures 
%.pdf : %.tex 
	@latexmk -pdf -output-directory=$(figdir) $< > /dev/null 

# compile latex with latexmk
$(MAIN).pdf: $(MAIN).tex $(figdir) $(FIGS) $(TABS) $(TIKZ) $(REF) *.tex Makefile
	@latexmk -pdf \
		-pdflatex="pdflatex --interaction=nonstopmode --shell-escape %O %S" \
		$(MAIN) > /dev/null

# list figure names 
listfigs : 
	@echo $(FIGS)

# list table names 
listtabs : 
	@echo $(TABS)

.PHONY : 
cleantikz : 
	@$(foreach file,$(basename $(TIKZ)),find . -maxdepth 1 -type f -name '$(file).*' ! -name '$(file).tex' -delete;)

# remove tex auxilary files 
.PHONY : clean 
clean : 
	latexmk -c 
	# rm -rf $(figdir) 
	rm -f $(MAIN).synctex.gz 
	rm -f $(MAIN).pdf
	rm -rf $(PYSRC)/__pycache__
	rm -rf __pycache__
	rm -f $(MAIN).spl 
	#rm -f $(MAIN).bbl
	rm -f $(MAIN).nav 
	rm -f $(MAIN).snm
	$(MAKE) cleantikz

==> figs/cp_4.tex <==
\newcommand{\sweepratiohone}{\num{3.0}\xspace} 
\newcommand{\sweepratiort}{\num{4.3}\xspace} 
\newcommand{\sweepratiohrt}{\num{6.6}\xspace} 
\newcommand{\rstdmax}{\num{42.6}\xspace} 
\newcommand{\rstdmin}{\num{9.9}\xspace} 

